Measurements of the Absolute Branching Fractions of $B^\pm \to K^\pm X_{c\bar c}$

A study of the two body decays $B^\pm\rightarrow X_{c\bar c}K^\pm$, where X$_{c\bar c}$ refers to one charmonium state, is reported by BaBar collaboration using a data sample of 424 fb$^{-1}$. The absolute determination of branching fractions for these decays are significantly improved compared to previous BaBaR measurements. Evidence is found for the decay $B^+\rightarrow X(3872)K^+$ at the $3\sigma$ level. The absolute branching fraction ${\cal B}(B^+\rightarrow X(3872)K^+) = (2.1\pm0.6({\rm stat})\pm0.3({\rm syst}))\times 10^{-4}$ is measured for the first time. It follows that ${\cal B}(X(3872)\rightarrow J/\psi\pi^+\pi^-)=(4.1\pm1.3)\%$, supporting the hypothesis of a molecular component for this resonance.

==> Definitions.tex <==

% Start of new 3Body definitions 
%
%  Definitions... link me from the cvs repo: 
%   BAD/3BDefn/Definitions.tex

%% Make sure xspace is loaded
\RequirePackage{xspace}

%% ---------------------------------------------------------- %%
%% General Commands
%% ---------------------------------------------------------- %%
%% Declare allowed hyphenation points
\hyphenation{brems-strahlung had-rons im-p-or-t-ant
             mis-iden-ti-fy mis-iden-ti-fied mis-iden-ti-fi-ca-tion}

%% ---------------------------------------------------------- %%
%% General Symbols
%% ---------------------------------------------------------- %%
\newcommand{\goto}{\rightarrow}
\newcommand{\calP}{\ensuremath{{\cal P}}}
\newcommand{\calH}{\ensuremath{{\cal H}}}
\newcommand{\pvec}{{\bf p}}
\newcommand{\pD}{\ensuremath{S}}		% for DIRC pulls
\newcommand{\thetac}{\ensuremath{\theta_C}}	% for the
				% Cherenkov angle
%% BF, charge asym, etc.
\newcommand{\acp}{\ensuremath{\calA_{ch}}}
\newcommand{\calB}{\ensuremath{{\cal B}}}
\newcommand{\signifSyst}{Signif. w syst. ($\sigma$)}
\newcommand{\corrEffB}{Corr. $\epsilon\times\prod\calB_i$ (\%)}
\newcommand{\prodB}{$\prod\calB_i$}
\newcommand{\bfemsix}{${\cal B}(10^{-6}$)}
\newcommand{\timesix}{\ensuremath{\times10^{-6}}}

%% tables
\newcommand\dbline{\noalign{\vskip 0.10truecm\hrule}\noalign{\vskip 2pt}\noalign{\hrule\vskip 0.10truecm}}
\providecommand{\tbline}{\noalign{\vskip 0.05truecm\hrule\vskip0.05truecm}}
\newcommand\sgline{\noalign{\vskip 0.10truecm\hrule\vskip 0.10truecm}}

%% f mesons 
\newcommand{\fzero}{\ensuremath{f_0}(980)\xspace}
\newcommand{\fzeros}{\ensuremath{f_0}\xspace}
\newcommand{\fzerop}{\ensuremath{f_0(1370)}\xspace}
\newcommand{\ftwo}{\ensuremath{f_2(1270)}\xspace}
\newcommand{\rhozero}{\ensuremath{\rho^0}\xspace}
%% K0s
\newcommand{\kzs}{\ensuremath{\KS}\xspace}
\newcommand{\kztopp}{\ensuremath{K^{0}\rightarrow K_S\rightarrow\pi^+\pi^-}\xspace}
\newcommand{\kstopipi}{\ensuremath{K^{0}_{S}\rightarrow\pi^+\pi^-}\xspace}
%% f0 K
\newcommand{\ffzeroK}{\ensuremath{\fzero\kaon}\xspace}
\newcommand{\fzeroK}{\ensuremath{\Bz\ra\ffzeroKs}}
\newcommand{\BfzeroK}{\ensuremath{\calB(\fzeroKs)}}
%% f0 Ks
\newcommand{\ffzeroKs}{\ensuremath{\fzero\KS}\xspace}
\newcommand{\ffzeroppKs}{\ensuremath{\fzero(\to\pi^+\pi^-)\KS}\xspace}
\newcommand{\ffzeropKs}{\ensuremath{\fzerop\KS}\xspace}
\newcommand{\frhozeroKs}{\ensuremath{\rhozero\KS}\xspace}
%
\newcommand{\fzeroKs}{\ensuremath{\Bz\ra\ffzeroKs}\xspace}
\newcommand{\fzeropKs}{\ensuremath{\Bz\ra\ffzeropKs}\xspace}
\newcommand{\rhozeropKs}{\ensuremath{\Bz\ra\frhozeropKs}\xspace}
%
% abbreviations
\newcommand{\fKs}{\ensuremath{fK_{\scriptscriptstyle S}}\xspace}
%% a00 K0

\newcommand{\razerozKz}{\ensuremath{xx^{+xx}_{-xx}\pm xx}}
\newcommand{\RazerozKz}{\ensuremath{(\razerozKz)\times 10^{-6}}\xspace}
\newcommand{\ulazerozKz}{\ensuremath{xx}\xspace}
\newcommand{\ULazerozKz}{\ensuremath{(\ulazerozKz)\times 10^{-6}}\xspace}
\newcommand{\sazerozKz}{\ensuremath{xx}\xspace}

%% ML fit (& other) variables
\newcommand{\Ebeam}{\ensuremath{E_{\rm beam}}}
\newcommand{\DE}{\ensuremath{\Delta E}}
\newcommand{\mb}{\ensuremath{m_{\rm ES}}}
%\newcommand{\mes}{\ensuremath{{m_{ES}}}}       % defined in babarsym.tex
\newcommand{\mres}{\ensuremath{m_{\rm res}}}
\newcommand{\xf}{\ensuremath{{\cal F}}}
\newcommand{\hel}{\ensuremath{{\cal H}}}
\newcommand{\thetaT}{\ensuremath{\theta_{\rm T}}}
\newcommand{\costhr}{\ensuremath{\cos\thetaT}}
\newcommand{\ctt}{\ensuremath{\costhr}}
\newcommand{\dEdx}{\ensuremath{\mathrm{d}E/\mathrm{d}x}}
\newcommand{\half}{\ensuremath{{1\over2}}}

%
% ----- definitions old 3 body stuff -----
%
\newcommand{\bei}{\begin{itemize}}
\newcommand{\eei}{\end{itemize}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\beqns}{\begin{eqnarray*}}
\newcommand{\eeqns}{\end{eqnarray*}}
\newcommand{\vs}{\\[0.3cm]\noindent}
\newcommand{\vssmall}{\\[0.15cm]\indent}
\newcommand{\vsn}{\\[0.3cm]\noindent}
\newcommand{\vsp}{\vspace{0.25cm}}
\newcommand{\vsm}{\vspace{-0.3cm}}
\newcommand{\hsm}{\hspace{-0.2cm}}
\newcommand{\hssm}{\hspace{-0.025cm}}
\newcommand{\intl}{\int\limits}
\newcommand{\ointl}{\oint\limits}
\newcommand{\mc}{\multicolumn}
\newcommand{\ph}{\phantom}
\newcommand{\e}{\epsilon}
%\newcommand{\hm}{\hspace{-0.1cm}}
\newcommand{\hmm}{\hspace{-0.2cm}}
\newcommand{\hmmm}{\hspace{-0.3cm}}
%
\def\bk{\!\!\!\!}
\def\rs{\raisebox{1.3ex}[-1.5ex]}
\def\TT{$\times10^{-3}$}
\def\tmsix{\times10^{-6}}
\def\tmthr{\times10^{-3}}
%
\newcommand{\GF}{G_{\rm F}}
\newcommand{\mee}{e^+e^-}
\def\MSbar{\overline{\rm MS}}
%
%...bibliography
\def\NP{{\em Nucl. Phys.}}
\def\PL{{\em Phys. Lett.}}
\def\PR{{\em Phys. Rev.}}
\def\PRep{{\em Phys. Rep.}}
\def\PRL{{\em Phys. Rev. Lett.}}
\def\NIM{{\em Nucl. Inst. Meth.}}
\def\ZP{{\em Z. Phys.}}
\def\CPC{{\em Comp. Phys. Comm.}}
\def\ea{{\em et al.}}
%\def\CoL{Collaboration}
%
%...stuff

\def\tho{{\rm theo}}
\def\exp{{\rm exp}}
\def\mod{{\rm mod}}
\def\QCD{{\rm QCD}}
\def\min{{\rm min}}
\def\max{{\rm max}}
\def\Min{{\rm Min}}
\def\Max{{\rm Max}}
%
% counts
\def\iA{I}
\def\iB{II}
\def\iC{III}
\def\iD{IV}
\def\iE{V}
\def\iF{VI}
\def\iG{VII}
\def\iH{VIII}
% B+ and B0
\def\bch{B$^pm$}
\def\bz{B$^0$}
%...trees and penguins
\def\TKpi{T_{K\pi}^{+-}}
\def\PKpi{P_{K\pi}^{+-}}
\def\PKzpi{P_{K\pi}^{0+}}
\def\Tpm{T^{+-}}
\def\Tmp{T^{-+}}
\def\Ppm{P^{+-}}
\def\Pmp{P^{-+}}
\def\Tzz{T^{00}}
\def\Tpz{T^{+0}}
\def\Tzp{T^{0+}}
\def\Pzz{P^{00}}
\def\Ppz{P^{+0}}
\def\Pzp{P^{0+}}
\def\rPTpm{r^{+-}}
\def\rPTmp{r^{-+}}
\def\rPTzz{r^{00}}
\def\rPTkappa{r^{\kappa}{}}
\def\rPTsigma{r^{\sigma}{}}
\def\rPTbarkappa{\kern 0.18em\overline{\kern -0.18em r}{}^{\kappa}{}}
\def\rPTbarsigma{\kern 0.18em\overline{\kern -0.18em r}{}^{\sigma}{}}
\def\deltapm{\delta_r^{+-}}
\def\deltamp{\delta_r^{-+}}
\def\deltazz{\delta_r^{00}}
\def\deltaTpm{\delta_T^{+-}}
\def\deltaTmp{\delta_T^{-+}}
\def\deltaTzz{\delta_T^{00}}
\def\deltakappa{\delta_r^{\kappa}}
\def\deltaTkappa{\delta_T^{\kappa}}
\def\deltasigma{\delta_r^{\sigma}}
\def\deltaTsigma{\delta_T^{\sigma}}
\def\deltabarkappa{\kern 0.18em\overline{\kern -0.18em \delta}{}_r^{\kappa}}
\def\deltabarsigma{\kern 0.18em\overline{\kern -0.18em \delta}{}_r^{\sigma}}
\def\deltaTbarkappa{\kern 0.18em\overline{\kern -0.18em \delta}{}_T^{\kappa}}
\def\deltaTbarsigma{\kern 0.18em\overline{\kern -0.18em \delta}{}_T^{\sigma}}
\def\phiTpm{\phi_T^{+-}}
\def\phiTmp{\phi_T^{-+}}
\def\phiTzz{\phi_T^{00}}

\def\Tpz{T^{+0}}
\def\Tcpz{T_C^{+0}}
\def\PpzEW{P^{+0}_{\rm EW}}
\def\PzpEW{P^{0+}_{\rm EW}}

\def\Tczz{T_C^{00}}
\def\Pzz{P^{00}}

\def\Aij{A^{ij}~}

\def\alphaeff{\alpha_{\rm eff}}
\def\thetarhopi{\theta}
%
% new for Dalitz
\def\OC{X}
\def\OCbar{{\kern 0.18em\overline{\kern -0.18em \OC}}}
\def\mBz{m_{\Bz}}
\def\spz{s_{+0}}
\def\smz{s_{-0}}
\def\spm{s_{+-}}
\def\mpz{m_{+0}}
\def\mmz{m_{-0}}
\def\mpm{m_{+-}}
\def\sab{s_{12}}
\def\sbc{s_{23}}
\def\sac{s_{31}}
\def\fpz{f_{+}}
\def\fmz{f_{-}}
\def\fpm{f_{0}}
\def\smzMax{{\smz}{}{[\rm max]}}
\def\smzMin{{\smz}{}{[\rm min]}}
\def\smzMaxMin{{\smz}{}{[\rm max/min]}}
\def\mpmMax{{\mpm}{}{[\rm max]}}
\def\mpmMin{{\mpm}{}{[\rm min]}}
\def\mpmMaxMin{{\mpm}{}{[\rm max/min]}}
\def\sbcMax{{\sbc}{}{[\rm max]}}
\def\sbcMin{{\sbc}{}{[\rm min]}}
\def\sbcMaxMin{{\sbc}{}{[\rm max/min]}}
\def\pipipi{\pip\pim\piz}
\def\Btopipipi{\Bz\to\pipipi}
\def\Btorhopi{\Bz\to\rho^\pm\pi^\mp}
\def\MatElm{{\cal M}(\Btopipipi)}
\def\mprime{m^\prime}
\def\thetaprime{\theta^\prime}
\def\deprime{{\de^\prime}{}}
\def\dt{\deltat}
\def\dterr{\sigma_{\deltat}}
\def\dtp{\Delta t^\prime}
\def\de{\DeltaE}
\def\demin{\de_{\rm min}}
\def\demax{\de_{\rm max}}
\def\mpmmax{{\mpm^{\rm max}}}
\def\NNprime{\NN^\prime}
\def\tpi{3\pi}
\def\Qeff{Q_{\rm eff}}
\def\Qeffi{Q_{{\rm eff},i}}
\def\Qtag{q_{\rm tag}}
\def\Qtagi{q_{{\rm tag},i}}
\def\Atagqq{A_{q\bar q,\,\rm tag}}
\def\Atag{A_{{B^+,\,\rm tag}}}
\def\Atagpj{A_{{B^+,\,\rm tag},j}}
\def\Atagzj{A_{{B^0,\,\rm tag},j}}
\def\cat{k}
\def\Amix{\ensuremath{A_{\rm mix}}}
\def\Amixc{\ensuremath{A_{{\rm mix},c}}}
\def\detJ{|\det J|}
\def\detJi{|\det J_i|}
\def\Rscf{R_{\rm SCF}}
\def\Rsqint{\e}
\def\DP{{\rm DP}}%
\def\dDP{d\DP}
\def\ampfrac{a}
\def\a{\kappa}
\def\b{\sigma}
\def\c{\tau}
\def\ab{\a\b}
\def\ac{\a\c}
\def\bc{\b\c}
\def\fitfrac{\eta}
\def\fitfracnorm{\hat\eta}
%
% new stuff
\def\kilo{{\rm k}}
%
% f0 KS
\newcommand{\Ham}{{\mathcal H}}
\newcommand{\HamIzero}{{\mathcal H}^{I=0}}
\newcommand{\HamIone}{{\mathcal H}^{I=1}}

\def\lambdabar{\kern 0.18em\overline{\kern -0.18em \lambda}}

\def\Abb{\kern 0.18em\overline{\kern -0.18em A}}
\def\Kbb{\kern 0.18em\overline{\kern -0.18em K}}

\def\AmpAll{{\cal A}_{\pi\pi\KS}}
\def\Appks{A_{\pi\pi\KS}}

\def\Afks{A_{\fzero\KS}}
\def\Afzerpks{A_{\fzero^\prime\KS}}
\def\Aftwoks{A_{f_2\KS}}
\def\Afkp{A_{\fzero\Kp}}
\def\Arhoks{A_{\rho^0\KS}}
\def\Afpks{A_{\fzero^\prime\KS}}
\def\Anr{A_{\rm NR}}

\def\Abppks{\Abb_{\pi\pi\KS}}

\def\Abfks    {\Abb_{\fzero\KS}}
\def\Abfzerpks{\Abb_{f_0^\prime\KS}}
\def\Abftwoks {\Abb_{f_2\KS}}
\def\Abrhoks  {\Abb_{\rho^0\KS}}
\def\Abfpks   {\Abb_{f_0^\prime\KS}}
\def\Abnr     {\Abb_{\rm NR}}

\def\Ffks{F_{\fzero\KS}}
\def\Frhoks{F_{\rho^0\KS}}
\def\Ffzeropks{F_{f_0^\prime\KS}}
\def\Fftwoks{F_{f_2\KS}}
\def\Ffpks{F_{f_0^\prime\KS}}
\def\Fnp{F_{\rm NP}}

\def\Tfks{T_{\fzero\KS}}
\def\Trhoks{T_{\rho^0\KS}}
\def\Tfpks{T_{\fzero^\prime\KS}}
\def\Tnp{T_{\rm NP}}
\def\Pfks{P_{\fzero\KS}}
\def\Prhoks{P_{\rho^0\KS}}
\def\Pfpks{P_{\fzero^\prime\KS}}
\def\Pnp{P_{\rm NP}}

\def\fprime{f_{0,2}^X}

\newcommand{\Sfzks}{\ensuremath S}
\newcommand{\Cfzks}{\ensuremath C}
%
% other new definitions
\def\logL{\log{\cal L}}
\def\R{{\rm Re}}
\def\I{{\rm Im}}
%
%...variables
\def\alphaSM{\alpha[{\rm SM}]}
\def\betaSM{\beta[{\rm SM}]}
\def\gammaSM{\gamma[{\rm SM}]}
\def\delpmmp{\hat\delta}
\def\lampm{\lambda^{+-}}
\def\lammp{\lambda^{-+}}
\def\lampmmp{\lambda^{+-(-+)}}
\def\kappm{\kappa^{+-}}
\def\kapmp{\kappa^{-+}}
\def\kappmmp{\kappa^{+-(-+)}}
\def\lamCP{\lambda_{\rm CP}}
\def\lamFL{\lambda_{\rm tag}}
\def\alphaeffpm{\alpha_{\rm eff}^{+-}}
\def\alphaeffpmmp{\alpha_{\rm eff}^{+-(-+)}}
\def\alphaeffmppm{\alpha_{\rm eff}^{-+(+-)}}
\def\alphaeffmp{\alpha_{\rm eff}^{-+}}
\def\alphaeffave{\alpha_{\rm eff}^{\pm}}
\def\bbar{\Bz \Bzb}
\def\Czz{C_{\rho\pi}^{00}}
\def\Szz{S_{\rho\pi}^{00}}
\def\Crhopi{C_{\rho\pi}}
\def\dCrhopi{\Delta C_{\rho\pi}}
\def\Cpizpiz{C_{\pi^0\pi^0}}
\def\Srhopi{S_{\rho\pi}}
\def\dSrhopi{\Delta S_{\rho\pi}}
\def\dS{\Delta S}
\def\dC{\Delta C}
\def\Acp{{\cal A}_{\rho\pi}}
\def\Acppz{{\cal A}_{\rho\pi}^{+0}}
\def\Acpzp{{\cal A}_{\rho\pi}^{0+}}
\def\Acppm{{\cal A}_{\rho\pi}^{+-}}
\def\Acpmp{{\cal A}_{\rho\pi}^{-+}}
\def\Acppmlim{|{\cal A}_{\rho\pi,}^{+-}|_{\rm max}}
\def\Acpmplim{|{\cal A}_{\rho\pi}^{-+}|_{\rm max}}
\def\Acpave{{{\cal A}_{\rho\pi}^\pm}}
\def\AcpKstrpi{{\cal A}_{K^*\pi}^{+-}}
\def\AcprhoK{{\cal A}_{\rho K}^{-+}}
\def\Npm{N^{+-}}
\def\Nmp{N^{-+}}
\def\Nbpm{{\kern 0.18em\overline{\kern -0.18em N}}^{+-}}
\def\Nbmp{{\kern 0.18em\overline{\kern -0.18em N}}^{-+}}
\def\rar{\rightarrow}
\def\rhoeta{(\bar\rho,\bar\eta)}
\def\rhobar{\bar\rho}
\def\etabar{\bar\eta}
\def\chisqmin{\chi^2_{\min}}
\def\sta{{\rm sin}\,2\alpha}
\def\staeff{{\rm sin}\,2\alphaeff}
\def\stb{{\rm sin}\,2\beta}
\def\stbb{{\rm sin}\,2\beta_{\rm BaBar}}
\def\stbwa{{\rm sin}\,2\beta_{\rm WA}}
\def\ttg{{\rm tan}\gamma}
\def\stastb{(\sta,\;\stb)}
\def\stagam{(\sta,\;\gamma)}
\def\stbgam{(\stb,\;\gamma)}
\def\stasq{{\rm sin}^22\alpha}
\def\stbsq{{\rm sin}^22\beta}
\def\ttgsq{{\rm tan}^2\gamma}
\def\sa{{\rm s}_{2\alpha}}
\def\sb{{\rm s}_{2\beta}}
\def\tg{{\rm t}_{\gamma}}
\def\sasq{{\rm s}^2_{2\alpha}}
\def\sbsq{{\rm s}^2_{2\beta}}
\def\tgsq{{\rm t}^2_{\gamma}}
\def\gam{\gamma}
\def\H{\rm H}
\def\xo{x_0}
\def\xobar{\bar\xo}
\def\xexp{x_{\exp}}
\def\xthe{x_{\tho}}
\def\ymod{y_{\mod}}
\def\ythe{y_{\tho}}
\def\yQCD{y_{\QCD}}
\def\yNP{y_{\rm NP}}
\def\Tthe{{\cal T}_{\tho}}
\def\sigexp{\sigma_{\exp}}
\def\sigxo{\sigma_o}
\def\Lik{{\cal L}}
\def\F{{\cal F}}
\def\U{{\mathfrak U}}
\def\C{{\mathfrak C}}
\def\T{{\mathfrak T}}
\def\Ndof{N_{\rm dof}}
\def\VCKM{{V}}
\def\CKM{{\rm CKM}}
\def\Likexp{{\cal L}_{\exp}}
\def\Likthe{{\cal L}_{\tho}}
\def\J{{J}}
\def\Mu{\mu}
\def\Chi2MinaMu{\chi^2_{\min ;\a,\Mu}}
\def\Chi2MinMu{\chi^2_{\min ;\Mu}(a)}
\def\Prob{{\cal P}}
\def\ProbCERN{{\rm Prob}}
\def\w{{\rm w}}
\def\Nthe{N_{\tho}}
\def\Nmod{N_{\mod}}
\def\NQCD{N_{\QCD}}
\def\Ncst{N_{\rm cst}}
\def\Neff{N_{\exp}^{\rm eff}}
\def\Na{N_{a}}
\def\Nmu{N_{\Mu}}
\def\Nexp{N_{\exp}}
\def\Nexpstar{N_{\exp}^\ast}
\def\NNP{N_{\rm NP}}
\def\Vubcb{\left|\frac{V_{ub}}{V_{cb}}\right|}
\def\VuboverVcb{|V_{ub}/V_{cb}|}
\def\Vubthe{|V_{ub}^\tho|}
\def\Vcbthe{|V_{cb}^\tho|}
\def\dmt{\Delta t}
\def\dmd{\Delta m_d}
\def\dms{\Delta m_s}
\def\DmBd{\dmd}
\def\DmBs{\dms}
\def\DmBdo{\Delta m_{B_d}^0}
\def\fbd{f_{B_d}}
\def\fbs{f_{B_s}}
\def\fbdbd{f_{B_d}\sqrt{B_d}}
\def\fbsbs{f_{B_s}\sqrt{B_s}}
\def\epsk{\epsilon_K}
\def\epe{\epsilon^\prime/\epsilon_K}
\def\kdo{{K^0-\bar{K^0}}}
\def\bdo{{B_d^0-\bar{B_d^0}}}
\def\bso{{B_s^0-\bar{B_s^0}}}
\def\CL{{\rm CL}}
\def\CLs{{\rm CL's}}
\def\CLcont{{\rm CL}_{\rm cont}}
\def\CLcut{{\rm CL}_{\rm cut}}
\def\Rzero{R_{\rm opt}}
\def\Rth{R_{\rm th}}
\def\xd{x_{\rm d}}
\def\xdo{x_{{\rm d}0}}
\def\corcof{{\rm c}}
\def\mec{\ensuremath{m_{\rm EC}}}
\def\costht{\ensuremath{|{\rm cos}(\theta_T)|}}
\def\cosmax{\ensuremath{|{\rm cos}_{\rm max}(\tilde\theta_T)|}}
\def\thrustEvent{{\hat T_{\rm Event}}}
\def\thrustB{{\hat T_B}}
\def\thrustRoe{{\hat T_\roe}}
\def\spherEvent{{\hat S_{\rm Event}}}
\def\spherB{{\hat S_B}}
\def\spherRoe{{\hat S_\roe}}
\def\pfirstRoe{{p^*_{\rm max,\,\roe}}}
\def\psecondRoe{{p^*_{\rm max2,\,\roe}}}
\def\cosBslow{{\rm cos}(\theta_{B_T,\pi({\rm slow})})}
\def\cosBfast{{\rm cos}(\theta_{B_T,\pi({\rm fast})})}
\def\sumpt{\Sigma_{p_T}}
\def\cerenkov{$\check{\rm C}{\rm erenkov}$ }
\def\xvar{{\cal X}}
\def\roe{{\rm ROE}}
\def\epso{\varepsilon_o}
\def\etao{\eta_o}
\def\epsc{\varepsilon_{\rm cut}}
\def\etac{\eta_{\rm cut}}
\def\epsMVA{\varepsilon_{_{\rm MVA}}}
\def\etaMVA{\eta_{_{\rm MVA}}}
\def\epst{\varepsilon_{\rm tot}}
\def\etat{\eta_{\rm tot}}
\def\boe{{\rm BOE}}
\def\pdf{\rm p.d.f}
\def\pdfs{\rm p.d.fs}
\def\MVA{\rm MVA}
\def\MVAs{\MVA s}
\def\GV{GV}
\def\PGV{pGV}
\def\NGV{nGV}
\def\FI{FI}
\def\NN{{\rm NN}}
\def\NNs{{\rm NNs}}
\def\TRU{{\rm TRU}}
\def\tru{{\rm tru}}
\def\TM{{\rm TM}}
\def\SCF{{\rm SCF}}
\def\scf{{\rm scf}}
\def\fscfave{\kern 0.18em\overline{\kern -0.18em f}_{\rm SCF}}
\def\fscf{f_{\rm SCF}}
\def\fscfi{f_{{\rm SCF},i}}
\def\Base{Base}
\def\BaseP{Base+}
\def\BasePP{Base++}
\def\ifb{{\rm fb}^{-1}}
\def\wbar {\ensuremath{\bar{w}}}
\def\avgD {\ensuremath{\langle D\rangle}}
\def\diffD {\ensuremath{\Delta D}}
\def\avgDcj {\ensuremath{\langle D\rangle^c_j}}
\def\diffDcj{\ensuremath{\Delta D^c_j}}
\def\cBtag{c}
\def\cBcp{c_{\rm CP}}
\def\pdf{\rm PDF}
\def\abar{\bar{a}}
\def\fBrhoplus {\ensuremath{f^{\rho^+\X^-}_{\Bz {\rm tag}}}}
\def\fBbarrhoplus {\ensuremath{f^{\rho^+\X^-}_{\Bzb {\rm tag}}}}
\def\fBrhominus {\ensuremath{f^{\rho^-\X^+}_{\Bz {\rm tag}}}}
\def\fBbarrhominus {\ensuremath{f^{\rho^-\X^+}_{\Bzb {\rm tag}}}}
\def\fBzxpm {\ensuremath{f^{\rho^\pm x^\mp}_{\Bz {\rm tag}}}}
\def\fBzbxpm {\ensuremath{f^{\rho^\pm x^\mp}_{\Bzb {\rm tag}}}}
\def\fBz {\ensuremath{f^{\pm}_{\Bz {\rm tag}}}}
\def\fBzb {\ensuremath{f^{\pm}_{\Bzb {\rm tag}}}}
\def\FBz {\ensuremath{F_{\Bz {\rm tag}}}}
\def\FBzb {\ensuremath{F_{\Bzb {\rm tag}}}}
\def\hel{{\theta_H}}
\def\cshelrho{{\rm cos}\hel(\rho)}
\def\cshelrhosq{{\rm cos}^2\hel(\rho)}
\def\cshelpiz{{\rm cos}\hel(\pi^0)}
\def\pfast{p_{\rm fast}^*}
\def\pslow{p_{\rm slow}^*}
\def\cosBmom{{\rm cos}\theta_{B,z}}
\def\cosBthr{{\rm cos}\theta_{T_B,z}}

\def\EPJ{{\em Eur. Phys. J.}}
\def\PRD{{\em Phys. Rev.}}
\def\PRL{{\em Phys. Rev. Lett.}}
\def\PL{{\em Phys. Lett.}}
\def\dalpha{\alpha-\alpha_{\rm eff}}

\def\BRpm{{\cal B}_{\rho\pi}^{+-}}
\def\BRmp{{\cal B}_{\rho\pi}^{-+}}
\def\Bbar{\kern 0.18em\overline{\kern -0.18em B}{}\xspace}

\def\BRpmb{{\cal \kern 0.18em\overline{\kern -0.18em  B}}{}_{\rho\pi}^{+-}}
\def\BRmpb{{\cal \kern 0.18em\overline{\kern -0.18em  B}}{}_{\rho\pi}^{-+}}
\def\BRipm{{\cal B}_{\rho^+\pi^-}}
\def\BRimp{{\cal B}_{\rho^-\pi^+}}
\def\BRipmb{{\cal \kern 0.18em\overline{\kern -0.18em  B}}{}_{\rho^+\pi^-}}
\def\BRimpb{{\cal \kern 0.18em\overline{\kern -0.18em  B}}{}_{\rho^-\pi^+}}
\def\BRall{{\cal B}_{\rho\pi}^{\pm\mp}}
\def\BRpmave{{\cal B}_{\rho\pi}^{\pm}}
\def\BRpz{{\cal B}_{\rho\pi}^{+0}}
\def\BRzp{{\cal B}_{\rho\pi}^{0+}}
\def\BRzz{{\cal B}_{\rho\pi}^{00}}
\def\BRrhoK{{\cal B}_{\rho K}^{-+}}
\def\BRKstrpi{{\cal B}_{K^*\pi}^{+-}}
\def\Abar{\kern 0.18em\overline{\kern -0.18em A}{}}
\def\abar{\kern 0.18em\overline{\kern -0.18em a}{}}
\def\apm{a^{+-}}
\def\amp{a^{-+}}
\def\apmb{\abar^{+-}}
\def\ampb{\abar^{-+}}
\def\Apm{A^{+-}}
\def\Amp{A^{-+}}
\def\Apmb{\Abar^{+-}}
\def\Ampb{\Abar^{-+}}
\def\Atpm{A_\prime^{+-}}
\def\Atmp{A_\prime^{-+}}
\def\Atpmb{\Abar_\prime^{+-}}
\def\Atmpb{\Abar_\prime^{-+}}
\def\Apz{A^{+0}}
\def\Amz{A^{-0}}
\def\Apzb{\Abar^{+0}}
\def\Azp{A^{0+}}
\def\Azpb{\Abar^{0+}}
\def\Azz{A^{00}}
\def\Azzb{\Abar^{00}}
\def\Apimpiz{A^{-0}}
\def\Apizpim{A^{0-}}
\def\AKpm{A_K^{+-}}
\def\AKmp{A_K^{-+}}
\def\TKpm{T_K^{+-}}
\def\TKmp{T_K^{-+}}
\def\PKpm{P_K^{+-}}
\def\PKmp{P_K^{-+}}
\def\Ppippim{P^{+-}}
\def\Ppimpip{P^{-+}}
\def\Ppippiz{P^{+0}}
\def\Ppizpip{P^{0+}}
\def\Pcalpm{{\cal P}^{+-}}
\def\Pcalmp{{\cal P}^{-+}}
\def\Pcalpz{{\cal P}^{+0}}
\def\Pcalzp{{\cal P}^{0+}}
\def\Pcalzz{{\cal P}^{00}}
\def\Ad{{A_{3/2,2}}}
\def\Ac{{A_{3/2,1}}}
\def\Ab{{A_{1/2,1}}}
\def\Aa{{A_{1/2,0}}}

% Major contribution from ChouxChef on 04 01 2001
% Name of the method -----------------------------
% default treatment
\def\rfit{{\em R}fit}
% extended treatment
% \def\ckmfoot{{\rm CKM}{\bf fit}$^{++}$~}
\def\erfit{{\em ER}fit}
% the package
\def\ckmfitter{{\em CKMfitter}}
\def\MINUIT{{\em MINUIT}}

%...latini
\def\ie{{\em i.e.}} 
\def\cf{{\em cf.}} 
\def\eg{{\em e.g.}} 
\def\via{via} 
\def\viz{{\em viz.}}

%...babar
%\def\babar{{B\footnotesize\hssm A\normalsize\hssm B\footnotesize\hssm AR}}
\def\babarEm{{\em B\footnotesize\em\hssm A\normalsize\em\hssm B\footnotesize\em\hssm AR}}
\def\babarBf{{\bf B\footnotesize\bf\hssm A\normalsize\bf\hssm B\footnotesize\bf\hssm AR}}

\def\ccbar{$c\overline{c}$~}
\def\cdbar{$c\overline{d}$~}
\def\cubar{$c\overline{u}$~}
\def\BBbar{$B\overline{B}$~}


\def\invfb{\ensuremath{\mbox{fb}^{-1}}\xspace} 
\def\ee{e^+e^-}
\def\mumu{\ensuremath{\mu^+\mu^-}\xspace}
\def\mm{\mu^+\mu^-}
\def\ll{\ell^+\ell^-}
\def\costh{\cos\theta}
\def\jHelCos{\costh_l}
\def\mrec{m_{rec}}
\def\pipiJ{\pi^+\pi^-  J/\psi}
\def\jee{\jp \rightarrow e^+e^-}
\def\jmm{\jp \rightarrow \mu^+\mu^-}
\def\jll{\jp \rightarrow \ell^+\ell^-}
\def\eff{\varepsilon}
\def\BR{{\cal B}}
\def\btoKX{B \rightarrow K X_{c\bar{c}}}
\def\Xcc{X_{c\bar{c}}}
\def\Lumi{{\cal L}}
\def\XsectV{\sigma_{\gamma\xspace V}}
\def\Gee{\Gamma_{V\to\,ee}}
\def\decay{\rightarrow}
\def\psipp{$\psi(3770)$}
\def\BaBar{\babar\xspace}
\def\psip{$\psi '$}
\def\Jpsi{J/$\psi$}
\def\etal{{\it et al.}}
\def\ccbar{$c\overline{c}~$}
\def\cdbar{$c\overline{d}~$}
\def\cubar{$c\overline{u}~$}
\def\BBbar{$B\overline{B}~$}
\def\hc{$h_c$}
\def\etac{$\eta_c$}
\def\etacp{$\eta_c (2S)$}
\def\chizero{$\chi_{c0}~$}
\def\chione{$\chi_{c1}~$}
\def\chitwo{$\chi_{c2}~$}
\def\bch{$B^\pm$}
\def\Kch{$K^\pm$}
\def\bz{$B^0$~}
\def\dz{$D^0$}
\def\ds{$D_s^\pm$}
\def\dch{$D^\pm$}
\def\dstar{$D^{*\pm}~$}
\def\dstarz{$D^{*0}~$}
\def\dstarzz{$D_1(2420)^0$~}
\def\dstarnew{$D^{**0}(2680)~$}

==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~A~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}

